Faithful Temporal Question Answering over Heterogeneous Sources

Temporal question answering (QA) involves time constraints, with phrases such as "... in 2019" or "... before COVID". In the former, time is an explicit condition, in the latter it is implicit. State-of-the-art methods have limitations along three dimensions. First, with neural inference, time constraints are merely soft-matched, giving room to invalid or inexplicable answers. Second, questions with implicit time are poorly supported. Third, answers come from a single source: either a knowledge base (KB) or a text corpus. We propose a temporal QA system that addresses these shortcomings. First, it enforces temporal constraints for faithful answering with tangible evidence. Second, it properly handles implicit questions. Third, it operates over heterogeneous sources, covering KB, text and web tables in a unified manner. The method has three stages: (i) understanding the question and its temporal conditions, (ii) retrieving evidence from all sources, and (iii) faithfully answering the question. As implicit questions are sparse in prior benchmarks, we introduce a principled method for generating diverse questions. Experiments show superior performance over a suite of baselines.

==> sections/09-ethics.tex <==
\section*{Ethical considerations}
\noindent Overall, we do not believe that this work has any negative societal impact.
On the contrary, we believe that enhancing the faithfulness and explainability of systems for knowledge-intensive tasks,
such as temporal QA systems,
can have a positive societal impact.
End users should have the possibility to understand how a system output was derived,
whether the output is faithful to the input, and thus whether the output can be
trusted or not.
% impact on society.
% There is a general consensus that systems for knowledge-intensive tasks,
% such as question answering,
% should be explainable.
% Explainability also requires being faithful to the 
% decide whether to trust
% or not trust a generated output.
% For knowledge-intensive tasks this includes the ability to provide traceable provenance for outputs,
% to give end users the 

% This paper tries to improve the faithfulness and explainability of temporal question answering.
% Our method aims to explain the answer derivation process to end users,
% and provides supporting evidence obtained from scrutable sources.
% Therefore, we believe that this work
% has a positive effect
% towards the general
% goal of explainable systems.

The \benchmark benchmark
presented in this paper
was
constructed using Wikipedia and Wikidata as input sources.
We did not make use of any personal or private data,
and did not involve crowdworkers.
% Whatever biases are there in the input data for constructing the question,
% might also be covered in the 
